It's not Easy: Applying Supervised Machine Learning to Detect Malicious Extensions in the Chrome Web Store

Google Chrome is the most popular Web browser. Users can customize it with extensions that enhance their browsing experience. The most well-known marketplace of such extensions is the Chrome Web Store (CWS). Developers can upload their extensions on the CWS, but such extensions are made available to users only after a vetting process carried out by Google itself. Unfortunately, some malicious extensions bypass such checks, putting the security and privacy of downstream browser extension users at risk. Here, we scrutinize the extent to which automated mechanisms reliant on supervised machine learning (ML) can be used to detect malicious extensions on the CWS. To this end, we first collect 7,140 malicious extensions published in 2017--2023. We combine this dataset with 63,598 benign extensions published or updated on the CWS before 2023, and we develop three supervised-ML-based classifiers. We show that, in a "lab setting", our classifiers work well (e.g., 98% accuracy). Then, we collect a more recent set of 35,462 extensions from the CWS, published or last updated in 2023, with unknown ground truth. We were eventually able to identify 68 malicious extensions that bypassed the vetting process of the CWS. However, our classifiers also reported >1k likely malicious extensions. Based on this finding (further supported with empirical evidence), we elucidate, for the first time, a strong concept drift effect on browser extensions. We also show that commercial detectors (e.g., VirusTotal) work poorly to detect known malicious extensions. Altogether, our results highlight that detecting malicious browser extensions is a fundamentally hard problem. This requires additional work both by the research community and by Google itself -- potentially by revising their approaches. In the meantime, we informed Google of our discoveries, and we release our artifacts.

==> commands.tex <==
\RequirePackage{listings}
\PassOptionsToPackage{hyphens}{url}\usepackage{hyperref}
%\usepackage{cite}
\usepackage{cleveref}
%\Crefformat{figure}{#2Fig.~#1#3}
\usepackage{listings}
\usepackage{stmaryrd}


\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\definecolor{eclipseStrings}{RGB}{42,0.0,255}
\definecolor{eclipseKeywords}{RGB}{127,0,85}
\colorlet{numb}{magenta!60!black}

\lstdefinelanguage{json}{
    commentstyle=\color{eclipseStrings}, % style of comment
    stringstyle=\color{eclipseKeywords}, % style of strings
    %numbers=left,
    %numberstyle=\scriptsize,
    %stepnumber=1,
    %numbersep=8pt,
    %showstringspaces=false,
    %breaklines=true,
    frame=lines,
    string=[s]{"}{"},
    comment=[l]{:\ "},
    morecomment=[l]{:"},
    literate=
        *{0}{{{\color{numb}0}}}{1}
         {1}{{{\color{numb}1}}}{1}
         {2}{{{\color{numb}2}}}{1}
         {3}{{{\color{numb}3}}}{1}
         {4}{{{\color{numb}4}}}{1}
         {5}{{{\color{numb}5}}}{1}
         {6}{{{\color{numb}6}}}{1}
         {7}{{{\color{numb}7}}}{1}
         {8}{{{\color{numb}8}}}{1}
         {9}{{{\color{numb}9}}}{1}
}

\lstdefinelanguage{JavaScript}{
    frame=lines,
  keywords={typeof, new, true, false, catch, function, return, null, catch, switch, var, if, in, while, do, else, case, break},
  ndkeywords={class, export, boolean, throw, implements, import, this},
  ndkeywordstyle=\color{darkgray},
  emph=[2]{postMessage, window.postMessage, chrome.runtime.sendMessage, chrome.runtime.connect, port.postMessage},
  emphstyle=[2]\color{blue},
  emph=[3]{window.onmessage, addEventListener, chrome.runtime.onMessage.addListener, chrome.runtime.onConnectExternal.addListener, p.onMessage.addListener},
  emphstyle=[3]\color{orange},
  sensitive=false,
  comment=[l]{//},
  morecomment=[s]{/*}{*/},
  morestring=[b]',
  morestring=[b]",
  alsoletter={.}
}

\lstset{ 
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
  basicstyle=\scriptsize,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  escapechar=\%,
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=single,	                   % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{red},       % keyword style
  language=JavaScript,                 % the language of the code
  morekeywords={typeof, new, true, false, catch, function, return, null, catch, switch, var, if, in, while, do, else, case, break, this},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,	                   % sets default tabsize to 2 spaces
  title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
}


\widowpenalty10000
\clubpenalty10000
\brokenpenalty=10000


\newcommand{\cmark}{{\textcolor{ACMGreen}{\ding{51}}\xspace}} % % TETC - pivoting
\newcommand{\xmark}{{\textcolor{ACMRed}{\ding{55}}\xspace}} % % TETC - pivoting

\newcolumntype{?}{!{\vrule width 1.5pt}}


\newcommand{\takeaway}[1]{
    \vspace{1em}
    \noindent\fbox{%
        \parbox{\columnwidth}{%
            \textbf{Takeaway}: {#1}
        }%
    }
}

\newcommand{\textbox}[1]{
    %\vspace{1em}
    \noindent\fbox{%
        \parbox{0.97\columnwidth}{%
            {#1}
        }%
    }
}

\newtcolorbox{cooltextbox}[1][]{%
    colback=black!5,
    colframe=black!5,
    notitle,
    sharp corners,
    % borderline west={1pt}{0pt}{red!80!black},
    borderline west={0pt}{0pt}{red!80!black},
    enhanced,
    breakable,
    left=0pt,
    right=0pt,
    top=0pt,
    bottom=0pt
    }


\newcommand\smamath[1]{{\small $#1$}}
\newcommand\smacal[1]{{\small $\mathcal{#1}$}}
\newcommand\smabb[1]{{\small $\mathbb{#1}$}}
\newcommand\normath[1]{$#1$}

\newcommand\ftbb[1]{{\footnotesize $\mathbb{#1}$}}
\newcommand\ftcal[1]{{\footnotesize $\mathcal{#1}$}}
\newcommand\ftmath[1]{{\footnotesize $#1$}}


\newcommand\scbb[1]{{\scriptsize $\mathbb{#1}$}}
\newcommand\sccal[1]{{\scriptsize $\mathcal{#1}$}}
\newcommand\scmath[1]{{\scriptsize $#1$}}


\newcommand{\todo}[1]{{\textcolor{red}{TODO: #1}}}
\newcommand{\af}[1]{{\textcolor{orange}{#1}}}
\newcommand{\ga}[1]{{\textcolor{blue}{#1}}}
\newcommand{\new}[1]{{\textcolor{black}{#1}}}
\newcommand{\tk}[1]{{\textcolor{black}{#1}}}

\newcommand{\jast}{\textsc{JaSt}}
\newcommand{\dx}{\textsc{DoubleX}}

\newcommand{\bigseta}{\texttt{{\Large Dataset L}}}
\newcommand{\bigsetb}{\texttt{{\Large Dataset U}}}

\newcommand{\smallseta}{\texttt{{\footnotesize Dataset L}}}
\newcommand{\smallsetb}{\texttt{{\footnotesize Dataset U}}}

\newcommand{\smallmeta}{\texttt{{\footnotesize Metadata classifier}}}
\newcommand{\smallcode}{\texttt{{\footnotesize Source code classifier}}}
\newcommand{\smallcomb}{\texttt{{\footnotesize Combined classifier}}}


\newcommand{\seta}{\texttt{Dataset L}}
\newcommand{\setb}{\texttt{Dataset U}}

\newcommand{\meta}{\texttt{Metadata classifier}}
\newcommand{\code}{\texttt{Source code classifier}}
\newcommand{\comb}{\texttt{Combined classifier}}


\newcommand{\pseudoparagraph}[1]{\vspace{2pt}\noindent\textbf{#1} ---}

\newcommand{\summary}[2]{
\vspace{0.5mm}
\textbox{
%{\small \textbf{{#1}} {#2}}
{\textbf{{#1}} {#2}}
}
}


% B
% Changes font size for \texttt
\makeatletter
% Definition of \ttfamily from latex.ltx
\DeclareRobustCommand\ttfamily
        {\not@math@alphabet\ttfamily\mathtt
         \fontfamily\ttdefault\small\selectfont}
\makeatother



